Mixture of Robust Experts (MoRE):A Robust Denoising Method towards multiple perturbations

To tackle the susceptibility of deep neural networks to adversarial examples, the adversarial training has been proposed which provides a notion of security through an inner maximization problem presenting the first-order adversaries embedded within the outer minimization of the training loss. To generalize the adversarial robustness over different perturbation types, the adversarial training method has been augmented with the improved inner maximization presenting a union of multiple perturbations e.g., various $\ell_p$ norm-bounded perturbations. However, the improved inner maximization only enjoys limited flexibility in terms of the allowable perturbation types. In this work, through a gating mechanism, we assemble a set of expert networks, each one either adversarially trained to deal with a particular perturbation type or normally trained for boosting accuracy on clean data. The gating module assigns weights dynamically to each expert to achieve superior accuracy under various data types e.g., adversarial examples, adverse weather perturbations, and clean input. In order to deal with the obfuscated gradients issue, the training of the gating module is conducted together with fine-tuning of the last fully connected layers of expert networks through adversarial training approach. Using extensive experiments, we show that our Mixture of Robust Experts (MoRE) approach enables a flexible integration of a broad range of robust experts with superior performance.

==> Sections/_Conclusion.tex <==
\section{Conclusion}


%The experimental results mentioned above generally demonstrate the robustness of our {\em MoRE} systems under different kinds of perturbations. Additionally, 

% As mentioned in the definition Hierarchically Gated {\em MoRE}, the first level of gating network in S2
% could make up the disadvantage of using structure S1 to mix clean experts with adversarial and natural perturbations robust training experts. In this section, we do a quick study to prove the rationality of make \emph{Softmax Weighted Gating} in the first gating layer of our Hierarchically Gated {\em MoRE}. The main inspiration of this method is came from the different weighted distribution of mixing clean expert with every different types of adversarially trained and robustly trained experts by using S1 when going through different training phase. The detailed values for CIFAR-10 and Tiny-ImageNet are both showed in Table~\ref{Weight_all_exp_cifar} and Table~\ref{Weight_all_exp_timage} in Appendix B. Since the main target of the first layer of Hierarchically Gated {\em MoRE} is
% to discriminate which types of images are feeding into the whole system, we could simplify the whole structure. The S1 structure with three experts (clean expert, $\ell_2$ adversarially trained expert with $\epsilon = 20/255$ and fog2 robustly trained expert) are adopted here. The values that are obtained by using CIFAR-10 is Table~\ref{Dtype_class_cifar}. And the weighted values of testing our classifier in Tiny-ImageNet is presented in Table~\ref{Dtype_class_timage}. As we can see, in each type, there is one expert dominate the weights especially in adversarial perturbation and natural perturbation type.
% The phenomenon also verifies our thought and demonstrate the rationality of introducing data type classifying gating module to the whole S1 {\em MoRE} systems as S2.

% Through the observing of these two tables, it indicates that the weighted value will have different distribution when figuring clean and different types of adversarial examples as well as natural perturbations into our S1 {\em MoRE} system. This property inspires us to the first general data type classifying gating layer to the S1 and finally got S2.
% we could simplify the structure of this part. It can only contain three experts that are belong to clean type expert, and most representative adversarial type as well as natural type experts. We select clean, $\ell_2$ adversarial training with $\epsilon = 80/255$ and fog2 as our final experts for Dynamic GT Classifier. 
% As we can see, in each type, there is one expert dominate the weights especially in adversarial perturbation and natural perturbation type.
% The phenomenon also verifies our thought and demonstrate the rationality of introducing data type classifying gating module to the whole S1 {\em MoRE} systems as S2. 

% not obtain the final accuracy We could 

% Compared with the classifying results of just using a single experts, our MoE systems could have robustness for various kinds of attacks without decreasing the performance of discriminating each type of images.  

% After obtaining these exciting results, for exploring in depth to understand why does this performance happen and develop the potential performance of our our MoE systems in mixing the various of experts, which are belong to totally different input types $T={clean, adversarial, natural}$. We need to give a deep exploration to out weighted values, which are the output of our weighted gate layer. The weighted values of our MoE systems under different training step are presented in Table~\ref{MoE_adv_w} and Table~\ref{MoE_nat_w}. Table~\ref{MoE_adv_w} are the weights output of implementing original MoE to clean experts and adversarial trained experts. And the Table~\ref{MoE_nat_w} are the weight value of implementing the MoE to clean experts and natural perturbations trained experts. 

%  Through observing these two tables, we could get a experimental facts basically. That fact is, when figuring a type of image to the whole MoE system, that weighted gate will put their primary focus on corresponding experts. As Table~\ref{MoE_adv_w}, the $\ell_p$ weighted value is obviously higher than clean experts when make their own attack type as input. Also, the weighted values of clean images are also higher than the $\ell_p$ adversarial trained experts when doing clean images training. 
% The similar weighted distributing phenomenon are also presented in Table~\ref{MoE_nat_w}. The weighted value of doing clean experts the maximal value among the five weighted values. Similarly, the fog/snow weighted values are also the maximal part when doing fog/snow perturbations training. 

==> Sections/ourmethod.tex <==
\section{Mixture of Robust Experts (\textit{\textbf{MoRE}}) Defense}\label{sec:methods}

{\em MoRE} (see Figures~\ref{fig_S1}) consists of three main components:
$1)$ expert models robust to a specific perturbation type, 
$2)$ trainable gating (or selection) mechanism to adaptively decide a combination of robust experts to process a given data sample, and
$3)$ efficient training approaches to optimize the robust experts and the gating module. 
%In this work, we explore two variants of gating modules resulting in two {\em MoRE} structures, S1 (Figure~\ref{fig_S1}) and S2 Figure~\ref{fig_S2}. 

In the following, we provide a detailed description of these components in the {\em MoRE} systems.

%Figure~\ref{fig_S1} demonstrates the structure S1, which uses a  weighted gating module to emphasize on the particular type of pretrained expert during the training of the whole ensemble learning system.
%After training each type of perturbations orderly and adopting Top-K loss optimization, the finally trained S1 structure could successfully defend against different types of perturbations. 
%For mixing all of experts together, in Figure~\ref{fig_S2}, Hierarchically Gated {\em MoRE} S2 is proposed. The structure of S2 is to add a first layer of gating module for input type classification. The first layer is to indicate which types of images are fed in the systems, namely adversarial examples, natural perturbations or clean inputs. %Then, we could use different {\em MoREs} separately for each type of inputs. 



\subsection{Robust Experts}

We use three different categories of experts: 1) an expert trained with the clean data, 
2) $N$ adversarial experts, each trained to be robust against a specific type of adversarial perturbation such as $\ell_p$ perturbations, and 
3) $N$ natural experts, each trained to be robust against a specific type of natural perturbation such as fog-perturbation and snow-perturbation. 
Details on how to train these experts are provided next. 


\noindent\textbf{Clean Expert.} The clean expert is trained using standard neural network training process with the clean training data $(x,y) \in \mathcal{D}_{clean}$.
The training process of the clean expert is as follows:
\begin{equation}
\label{eq:nature}
    \min_{\boldsymbol{\theta_c}} \quad \mathbb{E}_{(x,y) \sim \mathcal{D}_{clean}} [L(\boldsymbol{\theta_c},{x},{y}) ]
\end{equation}
where $\boldsymbol{\theta_c}$ denotes the model parameters, and $L$ is the cross entropy loss. 

\noindent\textbf{Adversarial Experts.} We use the adversarially trained experts to defend against adversarial perturbations. The robust (or min-max) optimization method~\citep{madry2018towards} is used to train experts to be robust under specific $\ell_p$-bounded adversarial attacks. The training process of the adversarial expert for a given $p$ is as follows:
\begin{equation}
\label{eq:minmax_adv}
    \min_{\boldsymbol{\theta_{adv}}} \,   \mathbb{E}_{({x},{y})\sim\mathcal{D}_{{clean}}}\left[\max_{\delta\in \boldsymbol{\Delta}_p }L(\boldsymbol{\theta_{adv}},{x}+\delta,{y})\right].
\end{equation}

With the clean data $\mathcal{D}_{clean}$, the inner maximization process aims to construct adversarial perturbation $\delta$ under $\ell_p$-ball constraint $\boldsymbol{\Delta}_p$, and then the outer minimization step aims to find model parameters $\boldsymbol{\theta_{adv}}$ robust to the generated adversarial examples.


\noindent\textbf{Natural Experts.} We also have the experts to be robust against various natural perturbations. 
For training these experts, we first transform the clean dataset $\mathcal{D}_{clean}$ to the natural perturbation dataset ${D}_{nat}$~\citep{ozdag2019susceptibility}. 
%The training process of these experts are similar as the adversarially trained experts. However, we need to replace the inner maximization step with a natural perturbations generating step. 
%By performing some mathematical manipulations, we could change the clean dataset $\mathcal{D}_{clean}$ to the data constituting natural perturbations ${D}_{nat}$~\cite{ozdag2019susceptibility}.
% \BK{Is there a paper we can cite that does adversarial training over natural perturbations? or we are doing just random data augmentation}
Then, the normal training process with  ${D}_{nat}$ is used to train the these experts with model parameters $\boldsymbol{\theta_{nat}}$. The training process for a given natural perturbation $i$ is as follows:
\begin{equation}
\label{eq:minmax_nat}
    \min_{\boldsymbol{\theta_{nat}}} \quad   \mathbb{E}_{({x}_{nat},{y})\sim\mathcal{D}_{nat}^i}\left[L(\boldsymbol{\theta_{nat}},{x}_{nat},{y})\right].
\end{equation}

%Adversarial attack is achieved by adding some imperceptible perturbations to the original image, however, this perturbation, which is generated by some mathematics measure, is so unnoticeable compared with original input but could make the DNN have a totally wrong prediction. The main purpose of doing research of network attacking is to discover some effective method to defend against this corresponding attack. 
%For adversarial attack, the most prevalent defensive method is to adopt Min-max robust optimization according to adversarial training method~\cite{madry2018towards}. Specifically, the inner maximization is used to simulate general attacking way, like PGD attack~\cite{madry2018towards}, and the outer minimization is an optimization process to train the whole model. These two steps could make the trained network ignore the influence of most attacks as much as possible, and make the defend against adversarial attack come true. 
%\textbf{Multi-task learning:} \\
%Through accomplishing the above steps, all pretrained experts could be obtained and placed into our two different kinds of MoE structures that will be introduced in Section 3.4. After completing the preparation of these three pretrained experts by using different general types of input images, our next step, which is also the major step of our algorithm, is to build the model structure of our Gating Module. Additionally, employing some approaches to accomplish the Efficient Training. And the General Types(GT) means three types including clean, adversarial and natural perturbations in this paper.  


% as presented in Figure 1. In the next training step of the MoE system, top K weighted Gate is introduced to determine the different weighting for each expert when classifying distinct images in the training process. 


\subsection{Gating Module}


%Another interesting feature of \emph{MoRE} is the presence of a gating mechanism that allows for specialization of experts in their respective domains. 
The aim of the trainable gating module (or selection mechanism) is to select an optimal combination of the experts to process each input and to decide how much weight to place on each expert for a given input. 
As opposed to traditional ensemble methods, e.g., stacking, that use constant weights based on an optimization criterion for the whole dataset, \emph{MoRE} dynamically estimates the weights through the gating network based on a given input data sample. As we will see later, this adaptability is specifically crucial in our setting where we are interested in achieving multiple otherwise conflicting objectives simultaneously. 

In this work, we explore two variants of gating networks in this paper (see Figures~\ref{fig_S1} and \ref{fig_S2}). Next, we explain common components in both  structures that are composed in different ways to design two gating mechanisms. 
Specifically, the two components of any gating network are: 1) Expert Gating, and 2) Weighting Mechanism.

\begin{wrapfigure}{r}{0.45\textwidth}
\centering
\includegraphics[scale=0.45]{figures/moe_new.pdf}
\caption{Framework for image classification using Gated \emph{MoRE} structure.}
\label{fig_S1}
\vspace{-8mm}
\end{wrapfigure}

\noindent\textbf{Expert Gating.}
Expert gating for a given set of robust experts is a network that acts as a feature extractor for a given image. 
This paper uses ResNet-18~{\citep{he2016deep}} for the trainable expert gating network architecture, with the output dimension equal to the number of given experts. 
We denote expert gating network as ${g}(\boldsymbol{\theta_g}; {x}_{i})$ where $\theta_g$ are trainable parameters.



\noindent\textbf{Weighting Mechanism.}
Having access to the gating network, we employ the following one weighting mechanisms:

\noindent \textit{1. Softmax Weighting:}
A choice of weighting is to apply the \emph{Softmax} function to expert gating to obtain the corresponding weight values of the experts for a specific image correspond to the $i$-th expert $\mathbf{x}_i$  
\begin{equation}
\label{eq:weight_gate}
       W = \textit{Softmax}\left({g}(\boldsymbol{\theta_g}; \mathbf{x}_{i})\right). 
\end{equation}

% \noindent \textit{2. Top-K Weighting:}
% To further improve the performance, we introduce sparsity in the weighting mechanism. In this weighting scheme, we filter out small weight values and only assign the top $K$ experts to an image. Specifically, before taking the \emph{Softmax} function, we only keep the $K$ highest values from the expert gating. We refer to this scheme as Top-K weighting mechanism

% \begin{equation}
% \label{eq:TK weight_gate exp}
% \begin{aligned}
%      & {W}_{TK} = \textit{Softmax}\left[TopK({g}(\boldsymbol{\theta_g}; \mathbf{x}_i), k)\right],  
% \end{aligned}
% \end{equation}
% where 
% \begin{eqnarray}
% \label{eq:TK weight_gate}
% TopK{(f,k)}_{i}=
% \begin{cases}
%  {y}_{i} & \text { if ${f}_{i}$ is in the top $k$ elements of $f$  } \\ 
%  -\infty & \text { otherwise}.
% \end{cases}
% \end{eqnarray}

% Having defined these components, we compose different variants of gating modules (and in turn \emph{MoRE} structures) as explained next.  
 
\subsection{Variants of {\textit{\textbf{MoRE}}} Structure}
\label{more}

Let us denote general data categories (e.g., clean, adversarial, and natural) using index $j \in \{1,\cdots,m\}$ and specific perturbations in these categories (e.g., $l_2$ and $l_\infty$ in adversarial data category) using index $i \in \{1,\cdots,n\}$. 
Also, let us denote robust expert specific to perturbation $i$ in general data category $j$ as $E_i^j$.
Next, we discuss two \emph{MoRE} structures used in the paper.

\subsubsection{\emph{MoRE}}
\label{more1}
% Top-K \emph{MoRE} structure comprises of a set of robust experts $\{E_i^j\}$ where $i \in \{1,\cdots,n\}$ and $j \in \{1,\cdots,m\}$. The gating module of Top-K \emph{MoRE} comprises of  expert gating for robust experts in set $\{E_i^j\}$ followed by Top-K weighting. The output of Top-K \emph{MoRE} is given by 

% \begin{equation}
% \label{eq:MoE}
% y = \sum_{j=1}^m\sum_{i=1}^n w_i^j E_i^j(\mathbf{x}_{i}),
% \end{equation}
% where $w_i^j$ corresponds to the weight for the respective expert in the vector $ W_{TK} = \textit{Softmax}\left[TopK({g}(\boldsymbol{\theta_g}; \mathbf{x_i}), k)\right]$.

% \begin{figure}[!t]
% \centering
% \includegraphics[scale=0.49]{figures/new_structure.pdf}
% \caption{Framework for image classification using Hierarchically Gated \emph{MoRE} structure.}
% \label{fig_S2}
% \end{figure}

% \subsubsection{Hierarchically Gated \emph{MoRE} (S2)}
\label{more1}
Our \emph{MoRE} structure comprises of a set of robust experts $\{E_i^j\}$ where $i \in \{1,\cdots,n\}$ and $j \in \{1,\cdots,m\}$. The gating module of Top-K \emph{MoRE} comprises of  expert gating for robust experts in set $\{E_i^j\}$ followed by different weights distribution. The output of our \emph{MoRE} is given by 

\begin{equation}
\label{eq:MoE}
y = \sum_{j=1}^m\sum_{i=1}^n w_i^j E_i^j(\mathbf{x}_{i}),
\end{equation}
where $w_i^j$ corresponds to the weight for the respective expert in the vector $ W_{TK} = \textit{Softmax}\left[{g}(\boldsymbol{\theta_g}; \mathbf{x_i})\right]$.



\subsection{Efficient Training Approaches}
\label{sec:more-train}
% Traditional ensemble learning methods are computationally \sout{very} expensive even with normal training and  performing a joint training of different experts and gating module along with min-max optimization will not be feasible in practice \LX{This sentence is too long}. 

Most of the traditional ensemble learning methods are computationally expensive even with the standard training. In the case of having different robust experts and gating modules, computationally more expensive min-max training will not be feasible in practice. 
Therefore, in this paper, we propose significantly more efficient approaches to train \emph{MoRE} structures. 
Next, we explain training approaches to (a) optimize the robust experts, and (b) optimize the gating module. 

Instead of training each layer of the robust experts jointly with gating module using the adversarial training, we propose to perform adversarial training of robust experts independently. This enables one to leverage embarrassingly parallel mechanism or even use pretrained robust experts. Given pretrained robust experts, the \emph{MoRE} training can be formulated as follows:  
\begin{equation}
    \label{more-train}
    \min_{\theta} \sum_{j=1}^m\sum_{i=1}^n\sum_{k=1}^K L( M_\theta(\mathbf{x}_i^j(k)),y_i^j(k))
\end{equation}
where $(\mathbf{x}_i^j(k)),y_i^j(k))$ denotes the $k$-th training samples of perturbation type $i$ from general data category $j$, $\theta_e = \{\theta_i^j\}_{i,j=1}^{n,m}$ denotes robust experts' last layer parameters (i.e., fine tuning), and $M_\theta$ denotes \emph{MoRE} as defined in Section~\ref{more}. Further, we have $\theta = \{\theta_e,\theta_g\}$ for our \emph{MoRE}.

We train the gating parameters along with robust experts' parameters by simple back-propagation. Note that we only fine tune robust experts' last fully connected layer $\theta_e$. As we will see next, this training process enjoys efficiency without loosing robustness or sacrificing accuracy. 


\BK{Gating parameters are now adversarially trained -- we need to mention that as in the last version is was normally trained.}

%\subsection{Mixture of Robust Experts ({\em MoRE}) Structure:}

%In practice, after obtaining the pretrained experts and the output of gating modules, we could combine these main constituent part and then form our {\em MoRE} system. Specifically, about the details of our ({\em MoRE}) structure, we introduce two different structures corresponding to different ensemble case. For Structure 1(S1), the application scenarios of this Structure is to mix one General Type($\ell_p$ adversarial examples or natural perturbations) with clean model. For example, a system mix one type of $\ell_p$ adversarial trained experts or one type of natural perturbations trained experts with clean images trained experts. This is a kind of S1 {\em MoRE} system. For Structure 2(S2), the main application scenarios of it is to mix different kinds of general type images with clean models. For example, a S2 {\em MoRE} system is able to mix clean experts, $\ell_p$ adversarial experts and natural perturbations trained experts together. The main difference between these two models is the S2 is created by introducing Dynamic Image Type Classifier to S1. In other words, S2 will consist the S1 in a way.


%\subsubsection{Structure 1 (S1):}
%As the information mentioned before, the main thought of our {\em MoRE} system is to mix weighted gating module and pretrained experts together. However, for the specific implementation of this thought, we need to solve two important issues about doing S1-{\em MoRE} training. 1) Obtaining the optimization object function consists of the pretrained experts and gating module items; 2) Define the whole S1 {\em MoRE} systems by using framework figure illustration.

%Concretely, in the case of already having experts and weighted values, the optimizing problem could be defined as the multiplication of each weighted value ${w}_{i}$ and the pretrained experts ${E}_{i}$. For mathematical representation, this output of the S1 could be described as following equation:

%\begin{equation}
%\label{eq:MoE}
%    %\min_{\boldsymbol{\theta}} \quad   
%   \hat{y} = \sum_{i}{w}_{i}{E}_{i}(\boldsymbol{\theta},{x}) \quad
%    i = 1, 2, \cdots, n
%\end{equation}
%After Introducing \eqref{eq:weight_gate} to this {\em MoRE} output equation, we can present the original optimizing problem as following equation:

%\begin{equation}
%\label{eq:MoE_gate}
%\begin{aligned}
%    & \min_{\boldsymbol{\theta_g},\boldsymbol{\theta_e}}    \sum_{i}{\textit{Softmax}\left({g}(\boldsymbol{\theta_g}\right)})_{i} \mathbb{E}_{i}\left[L(\boldsymbol{\theta_e},{x}_{i},{y}_{i})\right] \quad \\
    % &\min_{\boldsymbol{\theta}} \quad \sum_{i}{\textit{Softmax}\left[\mathbb{E}_{w} (L(\boldsymbol{\theta},{x}_{t},{y}_{t}) )\right]}_{i}\mathbb{E}_{i}\left[L(\boldsymbol{\theta},{x}_{i},{y}_{i})\right] \quad \\
%    & i = 1, 2, \cdots, n
%\end{aligned}
%\end{equation}
%where $\theta_e$ is the fine tuned parameters for all experts. 

%Furthermore, according to the analysis of the weighted distribution assigned by the gating module and some experiments study in the future section, we know that the whole S1 {\em MoRE} systems training process is actually dominated by some particular experts with the highest weighted value. Therefore, 
%introduce a kind of enhancing strategies to our initial Weighted Gating module and call our new methods as Top K weighted Gate.
%we introduce Top-k Gating to our original S1 {\em MoRE} systems and the optimization function could be  rewritten as the following format:


%  Through the structural analysis of our weight gate network and substantial experiments, we  Specifically, in the training process, instead of using all weight values generated by weighted gate, we will add a step to select the Top K values out of them. And just using these top K weighted value and their correspond experts as our actually used structures. This, our original MoE training function will be modified to have the following form:

%\begin{equation}
%\label{eq:MoE_gate_tk}
%\begin{aligned}
%    &\min_{\boldsymbol{\theta_g},\boldsymbol{\theta_e}} \quad  \emph{MoRE}_{topk}(\boldsymbol{\theta_g},\boldsymbol{\theta_{e}} ) = \\
%    &\sum_{i}{\textit{Softmax}\left(TopK({g}_{w}(\boldsymbol{\theta_g}), k)\right)}_{i}\mathbb{E}_{i}\left[L(\boldsymbol{\theta_{e}})\right] 
    % &\min_{\boldsymbol{\theta}} \quad \sum_{i}{\textit{Softmax}\left[\mathbb{E}_{w} (L(\boldsymbol{\theta},{x}_{t},{y}_{t}) )\right]}_{i}\mathbb{E}_{i}\left[L(\boldsymbol{\theta},{x}_{i},{y}_{i})\right] \quad \\
   %&i = 1, 2, \cdots, n
%\end{aligned}
%\end{equation}

%Where  $i = 1,2, ..., k$, through the definition of \eqref{eq:MoE_gate} and \eqref{eq:MoE_gate_tk}, the key problems that we need to solve now is define our S1 systems and know 
%how to optimize the whole structure legitimately. Our final model structure of S1 will be as Figure~\ref{fig_framework1}.
% \begin{equation}
% \label{eq:MoE_gate}
% \begin{aligned}
%     & \min_{\boldsymbol{\theta}} \quad   \sum_{i}{\textit{Softmax}\left({g}_{w}\right)}_{i}\mathbb{E}_{i}\left[L(\boldsymbol{\theta},{x}_{i},{y}_{i})\right] \quad 
%      i = 1, 2, \cdots, n \\
%     &\min_{\boldsymbol{\theta}} \quad \sum_{i}{\textit{Softmax}\left[\mathbb{E}_{w} (L(\boldsymbol{\theta},{x}_{t},{y}_{t}) )\right]}_{i}\mathbb{E}_{i}\left[L(\boldsymbol{\theta},{x}_{i},{y}_{i})\right] \quad 
% \end{aligned}
% \end{equation}

%\BK{What is this expectation on? Do we optimize $\theta$ or w}
%For the details of doing S1-{\em MoRE} training, in the beginning, these weights ${W}_{topk-w} = \{ {w}_{1}, {w}_{2}, \cdots, {w}_{n}\}$ are random initialized. However, after going through some epochs of the whole MoRE training, each expert ${E}_{i}$ will have their own specific weight ${w}_{i}$. These different weights make the whole MoRE know what is the proportion of its corresponding expert will constitute. Additionally, since each expert are all pretrained models, the main information of an expert has already been endowed. Therefore, in the training step of the whole MoRE systems, the major task is to find the appropriate weights to discriminate the different significance of each expert when figuring in different types of input.
%This task is totally different from the training goal of some current multi-task algorithms, which is to use training dataset to train all parameter and neuron in the training process.Our MoE systems just need to use training data to centralized train our weight gate, which is just a small part in our MoE system. For the remaining part of our MoRE, we just do fine-tuning to their last classifier layers. This operation could make each pretrained experts more suitable for the future MoRE systems. It will let the systems have better performance on achieving ensemble for classifying the images under different particular attacking types.

%\subsubsection{Structure 2 (S2)}

%After obtaining the initial structure and optimization strategy of S1, we aim to improve the performance of our final {\em MoRE} systems. There are some bad performance of S1 when mixing different CT and different PT experts together.Specifically, through analysing our model structure and the experimental results (Section 4), we discover that develop an effective defensive algorithm without decreasing clean accuracy is a very challenging research problem. Additionally, if we adopt S1 to mix different general types of experts, like mixing $\ell_p$ and one kind of natural perturbations experts synchronously, the final ensemble accuracy results will also be decreased in this situation. In order to overcome this drawbacks, we conduct some modifications to mix clean expert and different general types of experts(adversarial and natural perturbations) respectively. 

% Therefore, except for the clean trained models, the clean accuracy of other experts will all have various degree of decrease. 
%For solving the problems of S1 mentioned above, those two phenomena give us an insight to introduce a kind of input type classifier before figuring our input data to the S1-{\em MoRE}. Consequently, a pre-processing step of doing images general types classification named as Dynamic Image Types Classifier(DITC) will be added before S1. The main task of this classifier is to select the appropriate experts that we will use in the testing phase. The training phase of those S1 structure {\em MoRE} of CT and different PT will have similar optimization as \eqref{eq:MoE_gate}. However, the main contributions of DITC is on the testing phase. Instead of just labelling each clean and different GT of input images and achieve type classification by doing network training, we try to actualize in this classifier is to build the connection between the general types of pretrained experts and inputs images' types. This measure could maximally utilize the information of pretrained experts. The final output accuracy $Acc$ of our S2 in the testing pahse could be presented as following form:


%\begin{equation}
%\label{eq:MoE_gate}
%\begin{aligned}
%    & \quad \sum_{T}\emph{DITC}_{T} \times \emph{MoRE}_{topk}(\boldsymbol{\theta_g},\boldsymbol{\theta_{e}} )_{T} \\
    % &\min_{\boldsymbol{\theta}} \quad \sum_{i}{\textit{Softmax}\left[\mathbb{E}_{w} (L(\boldsymbol{\theta},{x}_{t},{y}_{t}) )\right]}_{i}\mathbb{E}_{i}\left[L(\boldsymbol{\theta},{x}_{i},{y}_{i})\right] \quad \\
    %& i = 1, 2, \cdots, n
%\end{aligned}
%\end{equation}

%Where $T$ indicates which type of {\em DITC} and {\em MoRE} will be used in S2. $T$ includes the CT and one of individual PT, such as $\ell_2$ adversarial type and fog type images.

% Concretely, our Structure 2(S2) is actually adding the Dynamic Image Type Classifier before figuring input images into different S1-{\em MoRE} systems.In addition, since the main task in this part is to discriminate different general types experts when using corresponding types of images to do model training, we could simplify our whole its structures when our S1-{\em MoRE} is used to do dynamic image type classification. For example, since the main types that we used in this paper are clean type, adversarial type and natural perturbations type, we could just select three different experts belong to these types individually to achieve out goal. 

% We could also testify the rationality of introducing Dynamic Image Type Classifier to our {\em MoRE} systems throug the observing the result in Section 4.The weighted value in Table~\ref{Dtype_class_cifar} prove the validity of our thought which means building the connection between types of inputs and the trained experts could achieving the function of classifying the experts' detailed types. The weighted value in Table~\ref{Dtype_class_cifar} prove the validity of our thought which means building the connection between types of inputs and the trained experts could achieving the function of classifying the experts' detailed types. Instead of labelling those three detailed types(clean, $\ell_2$ and fog) to the images, by using Top 1 weighted selection for the weighted Gate output, our Dynamic Image Type classifier will make the types of experts used in each testing process represent the corresponding input testing types. The rationality of this representing strategy could also be proven in Table~\ref{Dtype_class_cifar}, types of experts values is always the maximal one when doing the corresponding types of training. This method of doing images types classification could make the fully use of trained experts and do not need to waste or add too much extra steps for completing this types classifying process.

% \subsection{Dynamic Image type Classifier.}
% Through observing the results in Section 4.2 and Section 4.3. Our systems could introduce good classifying results improvement of doing ensemble to clean experts and another single type of attacking type, such as adversarial examples or natural perturbations. And for the internal of that single general type attack(adversarial or natural perturbations), our MoE system could also make the whole MoE system have the robustness enhancement for single similar or different sub-attacking type($\ell_2$, $\ell_\infty$; snow, fog). 


% However, the experimental results of applying the MoE or Top K MoE to all types of attacks ($T=$clean, adversarial, natural perturbations) mentioned above also present a disadvantage of our MoE systems. The ensemble results of these kinds of MoE is not so good despite these results is totally higher than just using single expert. In solving this kind of weakness, the weighted distribution in Table~\ref{MoE_adv_w} and Table~\ref{MoE_nat_w} give us a very good inspiration. Since the weighted value is dynamic distributed by which sub types of images are figuring into the systems. Therefore, we could make a dynamic sub type classifier of input images according to this weighted gate output property. 

% In those tables, we have obtained the experiments of applying MoE to five types of input(clean, $\ell_2$, $\ell_\infty$, fog and snow) and presented the related results. However, our experimental setting in this section is kind of different from the above experiments. The main parts that we need in our Dynamic Image Type Classifier is the output of Weighted Gate. And what we need to classify is that the testing input images is belong to which kind of general input types(clean, adversarial or natural). Consequently, we will select three types of models, which are the clean model as well as the representative model of adversarial and natural perturbations, to constitute the expert structure of our Dynamic Image Type Classifier. In detail, we adopt clean experts, $\ell_2$ with $\epsilon=80/255$ adversarial trained experts and fog trained experts(t = 0.13, light = 0.8) as the three experts of our model. Table~\ref{Dtype_class_cifar} give the weighted value of applying these three types of experts to our Top K MoE systems.



% general types of training dataset of each pretrained model and the inputs attacking types.In this paper, our general types are including clean, adversarial examples and natural perturbations, therefore, the expression MoE Selecting Gate is ${G}_{MoE} = \{ {w}_{clean}, {w}_{adv}, {w}_{nat}\}$. The model structure of this systems is presented in Figure~\ref{fig_framework2}.  \BK{This part is not clear, do you do 3 class classification? Also, image does not convey much information, you have 3 structures but only 2 figures}




% \begin{equation}
% \label{eq:MoE_K}
% \begin{aligned}
%     &\min_{\boldsymbol{\theta}} \quad   \sum_{i}{w}_{i}\mathbb{E}_{i}\left[L(\boldsymbol{\theta},{x}_{i},{y}_{i})\right] \quad 
%     i = 1, 2, \cdots, k\\ 
%      &\textit{s.t.} \quad {w}_{1} \textgreater {w}_{2} \textgreater
%      \cdots \textgreater {w}_{k} \textgreater \cdots \textgreater {w}_{n}
% \end{aligned}
% \end{equation}
% \BK{Optimization problem is not clear}
% This modification is intuitive in the algorithm design, however, this strategy is very useful for improving the efficiency of the algorithm. After introducing this strategy, the whole MoE systems just need to do fine-tuning for parts of the most important experts instead of optimizing the classifier layers of all experts. Additionally, the structure of our Top K  MoE systems is presented in Figure 2. 



% We first purpose a MoE structure called Top-K Mixture of Robust Experts (TK-MoRE) that is used to achieve the robustness against multiple perturbations simultaneously. The perturbations considered in this work not only include different $\ell_p$ perturbations but also  natural perturbations. The model structure of our TK-MoRE is presented in Figure~\ref{fig_framework}. The bulk of this structure is the $n$ Experts  ${\{E_i\vert i\;=\;1,\;\cdots,\;n\}}$ that are pretrained by different augmented data or adversarial training, and the Gate part $G$ is a kind of classifier that could output the weight value of different experts. The meaning of these weights is used to indicate the similarity of the expert's pretrained dataset and the input images. 

% In this paper, we obtain an ensemble systems that could defend against the $\ell_p$ adversarial attack and natural perturbations without decreasing the performance of classifying clean images that are not suffer any kinds of attacks. Therefore, each expert is a particular model to perform robust classification on a specific perturbation.

% \subsubsection{Structure 2:}


%The main part of this MoE selecting Gate is its weighted gate. The value of weighted gate allocated by 




% For each experts, each of them is a kind of CNN classifier to solve different tasks. 
% this task includes doing classification of clean images

% The 
% For MoE structure purposed in this paper, 

% that should try the whole systems from scratch. 




% \subsection{Top K Weighted Gate Module.}




% where $t$ indicates different types of input image, like ``clean", ``adversarial" or ``natural perturbations". \BK{What is $G_{weight}$ more information is needed}




% \subsection{Weighted Gate Training and Experts Fine-tuning}

% \begin{figure*}[tb]
% \begin{minipage}[b]{0.2\linewidth}
%   \centering
%   \centerline{\includegraphics[width=10cm]{figures/structure 1.pdf}}
% %  \vspace{1.5cm}
%   \centerline{(a)}\medskip
% \end{minipage}
% \hfill
% \caption{Structure 1.
% %Different kinds of triggers, (a)$y_t = 14$ (non-poisoned label); (b)$y_t = 38$ (non-poisoned label); (c) $y_t = 8$ (real-poisoned label); (d) original trigger with real poisoned label 8
% }
% \label{fig: fig1_example_backdoor}
% \end{figure*}



==> Sections/relatedwork.tex <==


\section{Related Work}\label{sec:related}

% \BK{We should start by highlighting that the problem of interest to the paper is achieving robustness to multiple perturbations and there are only a very few papers addressing this issues. So we first describe some related directions that focus on achieving robustness to just one perturbation and then discuss related work on multiple perturbations. We need to shorten this section as well -- as this may give an impression that there exist a lot of related work and baselines for MoRE which is not true.}
% Adversarial attack and defense as a topic to ensure the robustness of one model has been studied recently. And combining adversarial problem with ensemble learning, it a very fresh area in adversarial machine learning study. 
% \textcolor{green}{attacking}

% Adversarial Examples~\cite{szegedy2014intriguing}: Intriguing properties of neuralnetwork, ICLR2014

% C\&W Attack~\cite{carlini2017towards}: Towards evaluating the robustness of neural networks, SP2017

% Elastic-net attack~\cite{chen2018ead}: Elastic-net attacks to deep neural networks via adversarial examples, AAAI2018

% Structured Attack~\cite{xu2018structured}: Structured adversarial attack: Towards general implementation and better interpretability, ICLR 2019

% \textcolor{green}{defense}

% Adversarial Training~\cite{madry2018towards}, Towards deep learning models resistant to adversarial attacks, ICLR 2018


Although deep learning has achieved extraordinary performance in many application domains, it is well accepted that Deep Neural Networks (DNNs) are vulnerable under adversarial attacks \cite{szegedy2014intriguing}.
One major type of adversarial attacks is implemented by generating adversarial examples, which add imperceptible adversarial perturbations onto the original clean data with the purpose to fool DNN classifiers.
Representative adversarial attacks include C\&W attack \cite{carlini2017towards}, EAD attack \cite{chen2018ead}, Structured attack \cite{xu2018structured}, etc.
A principled approach to defend against a specific adversarial attack type is the adversarial training \cite{madry2018towards}, which formulates a min-max optimization problem to train a robust neural network, with the inner max problem modeling an universal first-order attack.
Furthermore, in response to the obfuscated gradients issue \cite{athalye2018obfuscated}, the adaptive attack has been investigated \cite{carlini2019evaluating}.


%\CH{ proposed an observation named obfuscated gradients, this gradient will happend in some defense method. They said this phenomenon will make some current adversarial defense perform a kind of false security since the defensive object of these method is not the optimal ones, they just circumvent the most powerful attacks intentionally or unintentionally. Therefore, for giving the new proposed model a more assured robust estimation, the adaptive attack are proposed to finish this task, including the simple adaptive attack and black box simba attack~\cite{guo2019simple}.}



This paper integrates ensemble learning with adversarial training as a more general and effective defense solution against a wide range of attacks. 
Therefore, this section reviews the related work on ensemble learning and its connection with adversarial machine learning.



\subsection{Ensemble Learning}

% Common ensemble learning~\cite{dietterich2000ensemble};
% Ensemble learning in Machine learning;
% International workshop on multiple classifier systems

% Majority Voting~\cite{polikar2012ensemble}
% Ensemble Learning;
% Ensemble machine learning

% Pareto multi-task~\cite{lin2019pareto};
% Pareto multi-task learning;
% NeurIPS.

% Multi-task Learning with dirichlet process~\cite{ xue2007multi};
% Multi-task learning for classification with dirichlet process priors;
% Journal of Machine Learning Research.

% Grouping and overlap in multi-task learning~\cite{kumar2012learning};
% Learning task grouping and overlap in multi-task learning;
% ICML.

% Quadratically gated MoE~\cite{liao2007quadratically};
% Quadratically gated mixture of experts for incomplete data classification;
% ICML 2007.


% Adaptive MoE~\cite{jacobs1991adaptive};
% Adaptive mixture of local experts;
% Neural computation.

% Life-long learning~\cite{aljundi2017expert};
% Expert gate: Lifelong learning with a network experts;
% CVPR 2017.




Ensemble learning combines the predictions from multiple machine learning models to improve the performance. 
Bagging and Boosting~\cite{dietterich2000ensemble, polikar2012ensemble} are examples of representative ensemble learning methods. 
Another important ensemble learning technique is Mixture-of-Experts (MoE)~\cite{liao2007quadratically,jacobs1991adaptive,aljundi2017expert}. MoE combines the outputs of several ``expert" models, each of which specializes on a different task. This is achieved by training a ``gating" module or selection mechanism that selects appropriate experts for a given input. MoE shows promise for building expressive models that are still cheap to compute at test time, and more parallelizable at training time.

\subsection{Ensemble Learning in Adversarial Machine Learning}


% Primary introduction, 
% \cite{tramer2017ensemble}, 
% Ensemble adversarial training: Attacks and defenses,
% ICLR

% Ensemble weak defense\cite{he2017adversarial}; 
% Adversarial example defense:Ensemble of weak defense are not strong.
% ;USENIX Workshop.


% Improving natural accuracy, \cite{saligrama2020revisiting},
% Revisiting Ensembles in an Adversarial Context: Improving Natural Accuracy, 
% ICLR Workshop


% Promoting Ensemble Diversity,\cite{pang2019improving}, 
% Improving Adversarial Robustness via Promoting Ensemble Diversity, ICML 2019

% multi-task learning, \cite{maini2019adversarial};
% Adversarial robustness against the union of perturbation models,
% ICML 2019

% Max and Average training, \cite{tramer2019adversarial}, Adversarial training and robustness for multiple perturbations,
% NIPS 2019

% Classify Then Predict (CTP),\cite{Pratyush2020multiple} Classifying Perturbation Types for Robustness
% Against Multiple Adversarial Perturbations, UDL2020



% ----------------------------------
% \textcolor{red}{I agree to BK that this section is unnecessarily long. Please introduce one paper with 2-3 sentences. And don't need to use sentences in between papers as transitions, we are not a survey paper, OK?}


With an increasing interest on adversarial attacks and defenses of DNNs, ensemble learning techniques have also been applied in the adversarial machine learning setting from both the defense and attack perspectives.


% \textcolor{yellow}{Hao, I reordered the above list. Talk about the papers according to the above order.}

% Originally, the tasks of ensemble learning in adversarial case are just similar as the normal case.

Ensemble Adversarial training \cite{tramer2017ensemble} is a technique to augment training data with stronger perturbations transferred from other models. Specifically, the benefit of ensemble adversarial training is that it increases the diversity of adversarial examples so that the model can fully explore the adversarial example space. 


Another task that is achieved using ensemble learning is to make defense maintain a better performance in clean input case.
Specifically, \cite{saligrama2020revisiting} use two schemes, one that averages the predictions from several randomly initialized robust
models, and the other that also use average to fuse features from robust and standard model, to increase their clean accuracy in adversarial training.  
Further, \cite{he2017adversarial} uses ensemble learning to combine the predictions of weak defenses. They showed that an ensemble of weak defenses is not sufficient to provide strong defense against adversarial examples.
Pang et al. \cite{pang2019improving} introduced a method to increase the diversity of resulting ensemble by employing the ensemble diversity. Specifically, they propose Adaptive Diversity Promoting (ADP) regularizer to be used with the training loss. The authors show that their methods leads to globally better robustness for the ensemble by making adversarial examples difficult to transfer among individual members. 



All of these approaches discussed above focus on improving the robustness to a specific adversarial attack type.
Another promising research direction is adopting ensemble learning to enhance the DNN's robustness to a broad range of attacks. This has achieved some attention recently. 





The authors in \cite{tramer2019adversarial} study the trade-offs of adversarial robustness in various settings when defending against aggregations of multiple adversaries. They proposed aggregation of different adversaries for adversarial training against multiple perturbation models. Specifically, Max and Average strategies were proposed to achieve this. Max strategy trains the model on the strongest adversarial example from all the attacks. Average strategy, on the other hand, simultaneously trains on adversarial examples from all attacks. 
The authors in \cite{maini2019adversarial} notices that existing schemes tend to converge to suboptimal local minima, resulting in a model that is highly robust to certain perturbation models while failing to defend against others.
Thus, they proposed {Multi Steepest Descent (MSD)} to achieve a better performance. 
MSD generates adversarial examples for augmentation by taking the worst-case over all steepest descent directions. This approach has the advantage of directly converging upon a trade-off between different perturbation models which minimizes the worst-case performance over the union. To improve the robustness to multiple perturbation types, a concurrent work \cite{Pratyush2020multiple} proposed simple Classify Then Predict (CTP) scheme. CTP first classifies the perturbation type of the input, and then leverages a label predictor specifically trained against that adversary to provide the final prediction.



% define a new notion of ensemble diversity in adversarial setting and try to encourage the diversity of their systems by adopting an adaptive diversity promoting (ADP) regularizer to train their whole model. After the ADP regularizer training, the ensemble trainied model could have the diverse robust for different perturbations and achieve the defense against different attacks.


% Currently, most of adversarial attacks adopt PGD attack as their attacking type currently. Therefore,  in designing the systems with different robustness for different types of attacks
% \textcolor{blue}{changed}


% In this research direction, \cite{tramer2019adversarial} propose the detailed application of applying Ensemble Adversarial Training to generate one model could defend against different types of $l_p$ adversarial examples. The main modified process is still the data augmentation. And in the concrete training step, they firstly obtain the loss value that are forward computed by different types of adversarial examples. And then achieve the back-propagation by using the a final loss calculated by adopting MAX or AVERAGE operation to different types of loss. The final Ensemble Adversarial Trained model could achieve the model robust for those perturbations that have been added to the training dataset. 


%This method is an attack as well as a defense. 

% In each attack step, it calculates the losses for different perturbation models, the gradients with respect to a input image, and the perturbations for the image. Next, it compares the different losses, and chooses the perturbation with the maximum loss value. Currently, this method could only be applied to projected gradient descent (PGD) adversarial method; therefore, we cannot apply this method to natural perturbations. We compare the result in section 4.








% method to defend against the different perturbations that are generated by one type of attacking method with different types of bounding box($\ell_1$, $\ell_2$ and $\ell_\infty$) \textcolor{blue}{Where comes the bounding box?}


% Even the work about this topic is inadequate now, there are still some methods that are proposed to solve this question. 



